Excitation Trajectory Optimization for Dynamic Parameter Identification Using Virtual Constraints in Hands-on Robotic System

This paper proposes a novel, more computationally efficient method for optimizing robot excitation trajectories for dynamic parameter identification, emphasizing self-collision avoidance. This addresses the system identification challenges for getting high-quality training data associated with co-manipulated robotic arms that can be equipped with a variety of tools, a common scenario in industrial but also clinical and research contexts. Utilizing the Unified Robotics Description Format (URDF) to implement a symbolic Python implementation of the Recursive Newton-Euler Algorithm (RNEA), the approach aids in dynamically estimating parameters such as inertia using regression analyses on data from real robots. The excitation trajectory was evaluated and achieved on par criteria when compared to state-of-the-art reported results which didn't consider self-collision and tool calibrations. Furthermore, physical Human-Robot Interaction (pHRI) admittance control experiments were conducted in a surgical context to evaluate the derived inverse dynamics model showing a 30.1\% workload reduction by the NASA TLX questionnaire.

==> old-table.tex <==
\begin{comment}
\begin{table*}[t]
\centering
\caption{NASA-TLX Table for the shared docking task}
\label{table1}
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Dimension (weight)}} & \multicolumn{4}{c|}{\textbf{Score (0-100), lower is best}} \\ \cline{2-5} 
 & \textbf{Experimental Group} & \textbf{Control Group (CG)} & \textbf{Experimental Group} & \textbf{CG with tool calibration} \\ \hline
Mental Demand (0.2) & $12.70\pm 5.85$&$63.80\pm 19.34$& $18.10\pm 16.58$ & $21.80\pm 21.94$ \\ \hline
Physical Demand (0.2) & $12.50\pm 6.12$& $65.00\pm17.53$& $13.20 \pm 10.60$ & $22.70\pm 21.84$\\ \hline
Temporal Demand (0.1) & $19.90\pm 14.56$& $53.40\pm 27.63$& $17.20 \pm 13.27$&$23.40\pm 20.32$\\ \hline
Performance (0.2) & $14.50\pm 9.53$&$63.70\pm 19.88$& 
$15.90 \pm 9.79$&$23.60\pm 19.18$ \\ \hline
Effort (0.2) & $18.80\pm 9.39$& $58.90\pm 16.65$&
$15.20 \pm 9.02$&$22.60\pm 19.11$\\ \hline
Frustration Level (0.1) & $13.50\pm 7.43$&$55.20\pm 24.06$&
$15.20 \pm 10.28$&$21.70\pm 18.08$ \\ \hline
\textbf{Total NASA TLX Score} & $15.04\pm 8.38$& $61.14\pm 19.85$&
$15.72 \pm 11.55$&$22.65\pm 20.56$ \\ \hline
\end{tabular}
\vspace{-10pt}
\end{table*}
\end{comment}
